Scale-invariant Bayesian Neural Networks with Connectivity Tangent Kernel

Explaining generalizations and preventing over-confident predictions are central goals of studies on the loss landscape of neural networks. Flatness, defined as loss invariability on perturbations of a pre-trained solution, is widely accepted as a predictor of generalization in this context. However, the problem that flatness and generalization bounds can be changed arbitrarily according to the scale of a parameter was pointed out, and previous studies partially solved the problem with restrictions: Counter-intuitively, their generalization bounds were still variant for the function-preserving parameter scaling transformation or limited only to an impractical network structure. As a more fundamental solution, we propose new prior and posterior distributions invariant to scaling transformations by \textit{decomposing} the scale and connectivity of parameters, thereby allowing the resulting generalization bound to describe the generalizability of a broad class of networks with the more practical class of transformations such as weight decay with batch normalization. We also show that the above issue adversely affects the uncertainty calibration of Laplace approximation and propose a solution using our invariant posterior. We empirically demonstrate our posterior provides effective flatness and calibration measures with low complexity in such a practical parameter transformation case, supporting its practical effectiveness in line with our rationale.

==> fig/1d_reg.tex <==
\begin{figure*}[!t]
    \centering
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_reg/ntkgp_relu.pdf}
        \captionsetup{justification=centering}
        \caption{LL / ReLU ($\alpha=$100.0)}
        \label{fig:ll_step_0}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_relu_priors/0.01.pdf}
        \captionsetup{justification=centering}
        \caption{LL / ReLU ($\alpha=$0.01)}
        \label{fig:ll_step_100}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_reg/ctkgp_relu.pdf}
        \captionsetup{justification=centering}
        \caption{CL / ReLU ($\alpha=$100.0)}
        \label{fig:cl_step_0}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_relu_priors_cl/1.0.pdf}
        \captionsetup{justification=centering}
        \caption{CL / ReLU ($\alpha=$1.0)}
        \label{fig:cl_step_100}
    \end{subfigure}
    \caption{\footnotesize Toy 1D regression task for Linearized Laplace (LL) and Connectivity Laplace (CL). We plot ground truth (black), training data (blue), predictive mean (red), and predictive uncertainty (shaded area). We provide two scales of prior for each method: One scale matches to the weight decay coefficient and the other scale capture both 'in-between' uncertainty \cite{foong2019between} and out-of-distribution uncertainty. We refer to Appendix~\ref{supp:various-prior-scale} for results for various prior scales.}
    \label{fig:1d-reg}
    \vspace{-0.5cm}
\end{figure*}

==> fig/1d_reg_wo_bn.tex <==
\begin{figure*}[!ht]
    \centering
    \begin{subfigure}[h]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_reg_wo_bn/ntkgp_relu.pdf}
        \captionsetup{justification=centering}
        \caption{LL / ReLU}
    \end{subfigure}
    \begin{subfigure}[h]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_reg_wo_bn/ntkgp_tanh.pdf}
        \captionsetup{justification=centering}
        \caption{LL / TanH}
    \end{subfigure}
    \begin{subfigure}[h]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_reg_wo_bn/ctkgp_relu.pdf}
        \captionsetup{justification=centering}
        \caption{CL / ReLU}
    \end{subfigure}
    \begin{subfigure}[h]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_reg_wo_bn/ctkgp_tanh.pdf}
        \captionsetup{justification=centering}
        \caption{CL / TanH}
    \end{subfigure}
    \caption{Toy 1D regression task for Linearized Laplace (LL) and Connectivity Laplace (CL) without BN. We plot ground truth (dotted black line), predictive mean (red line), and predictive uncertainty (shaded area). Blue points indicate the training samples.}
\end{figure*}

==> fig/1d_reg_wo_wd.tex <==
\begin{figure*}[!ht]
    \centering
    \begin{subfigure}[h]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_reg_wo_wd/ntkgp_relu.pdf}
        \captionsetup{justification=centering}
        \caption{LL / ReLU}
    \end{subfigure}
    \begin{subfigure}[h]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_reg_wo_wd/ntkgp_tanh.pdf}
        \captionsetup{justification=centering}
        \caption{LL / TanH}
    \end{subfigure}
    \begin{subfigure}[h]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_reg_wo_wd/ctkgp_relu.pdf}
        \captionsetup{justification=centering}
        \caption{CL / ReLU}
    \end{subfigure}
    \begin{subfigure}[h]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_reg_wo_wd/ctkgp_tanh.pdf}
        \captionsetup{justification=centering}
        \caption{CL / TanH}
    \end{subfigure}
    \caption{Toy 1D regression task for Linearized Laplace (LL) and Connectivity Laplace (CL) without weight decay. We plot ground truth (dotted black line), predictive mean (red line), and predictive uncertainty (shaded area). Blue points indicate the training samples.}
\end{figure*}

==> fig/1d_relu_priors.tex <==
\begin{figure*}[!h]
    \centering
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_relu_priors/0.001.pdf}
        \captionsetup{justification=centering}
        \caption{LL / ReLU (1e-3)}
        \label{fig:ll_relu_1e-3}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_relu_priors/0.01.pdf}
        \captionsetup{justification=centering}
        \caption{LL / ReLU (1e-2)}
        \label{fig:ll_relu_1e-2}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_relu_priors/0.1.pdf}
        \captionsetup{justification=centering}
        \caption{LL / ReLU (1e-1)}
        \label{fig:ll_relu_1e-1}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_relu_priors/1.0.pdf}
        \captionsetup{justification=centering}
        \caption{LL / ReLU (1e-0)}
        \label{fig:ll_relu_1e-0}
    \end{subfigure}
    \caption{Toy 1D regression task for Linearized Laplace (LL) for various prior scales. Results show that LL with small prior scale (1e-3) fails to capture 'in-between' uncertainty \cite{foong2019between}. On the other hand, LL with large prior scale (>=1e-2) suffers from under-fitting issue.}
    \label{fig:1d-relu_hparams}
\end{figure*}

==> fig/1d_relu_priors_cl.tex <==
\begin{figure*}[!h]
    \centering
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_relu_priors_cl/0.1.pdf}
        \captionsetup{justification=centering}
        \caption{CL / ReLU (1e-1)}
        \label{fig:cl_relu_1e-1}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_relu_priors_cl/1.0.pdf}
        \captionsetup{justification=centering}
        \caption{CL / ReLU (1e-0)}
        \label{fig:cl_relu_1e-0}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_relu_priors_cl/10.0.pdf}
        \captionsetup{justification=centering}
        \caption{CL / ReLU (1e+1)}
        \label{fig:cl_relu_1e+1}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_relu_priors_cl/100.0.pdf}
        \captionsetup{justification=centering}
        \caption{CL / ReLU (1e+2)}
        \label{fig:cl_relu_1e+2}
    \end{subfigure}
    \caption{Toy 1D regression task for Connectivity Laplace (CL) for various prior scales. While CL with small prior scale (<=1e-1) fail to capture 'in-between' uncertainty\cite{foong2019between}, CL with large prior scale (>1e-1) does not suffer from under-fitting issue.}
    \label{fig:1d-relu_hparams_cl}
\end{figure*}

==> fig/1d_relu_sigma.tex <==
\begin{figure*}[!h]
    \centering
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_relu_sigma/0.001.pdf}
        \captionsetup{justification=centering}
        \caption{LL / ReLU (1e-3)}
        \label{fig:ll_relu_1e-3_sigma}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_relu_sigma/0.01.pdf}
        \captionsetup{justification=centering}
        \caption{LL / ReLU (1e-2)}
        \label{fig:ll_relu_1e-2_sigma}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_relu_sigma/0.1.pdf}
        \captionsetup{justification=centering}
        \caption{LL / ReLU (1e-1)}
        \label{fig:ll_relu_1e-1_sigma}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_relu_sigma/1.0.pdf}
        \captionsetup{justification=centering}
        \caption{LL / ReLU (1e-0)}
        \label{fig:ll_relu_1e-0_sigma}
    \end{subfigure}
    \caption{Toy 1D regression task for Linearized Laplace (LL) for various prior scales. Results show that LL with small prior scale (1e-3) fails to capture 'in-between' uncertainty \cite{foong2019between}. On the other hand, LL with large prior scale (>=1e-2) suffers from under-fitting issue.}
    \label{fig:1d-relu_sigma}
\end{figure*}

==> fig/1d_relu_sigma_cl.tex <==
\begin{figure*}[!h]
    \centering
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_relu_sigma_cl/0.1.pdf}
        \captionsetup{justification=centering}
        \caption{CL / ReLU (1e-1)}
        \label{fig:cl_relu_1e-1_sigma}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_relu_sigma_cl/1.0.pdf}
        \captionsetup{justification=centering}
        \caption{CL / ReLU (1e-0)}
        \label{fig:cl_relu_1e-0_sigma}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_relu_sigma_cl/10.0.pdf}
        \captionsetup{justification=centering}
        \caption{CL / ReLU (1e+1)}
        \label{fig:cl_relu_1e+1_sigma}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_relu_sigma_cl/100.0.pdf}
        \captionsetup{justification=centering}
        \caption{CL / ReLU (1e+2)}
        \label{fig:cl_relu_1e+2_sigma}
    \end{subfigure}
    \caption{Toy 1D regression task for Connectivity Laplace (CL) for various prior scales. While CL with small prior scale (<=1e-1) fail to capture 'in-between' uncertainty\cite{foong2019between}, CL with large prior scale (>1e-1) does not suffer from under-fitting issue.}
    \label{fig:1d-relu_hparams_cl}
\end{figure*}

==> fig/1d_tanh_priors.tex <==
\begin{figure*}[!h]
    \centering
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_tanh_priors/0.001.pdf}
        \captionsetup{justification=centering}
        \caption{LL / TanH (1e-3)}
        \label{fig:ll_tanh_1e-3}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_tanh_priors/0.01.pdf}
        \captionsetup{justification=centering}
        \caption{LL / TanH (1e-2)}
        \label{fig:ll_tanh_1e-2}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_tanh_priors/0.1.pdf}
        \captionsetup{justification=centering}
        \caption{LL / TanH (1e-1)}
        \label{fig:ll_tanh_1e-1}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_tanh_priors/1.0.pdf}
        \captionsetup{justification=centering}
        \caption{LL / TanH (1e-0)}
        \label{fig:ll_tanh_1e-0}
    \end{subfigure}
    \caption{Toy 1D regression task for Linearized Laplace (LL) for various prior scales. Results show that LL with small prior scale (<=1e-2) fails to capture 'in-between' uncertainty \cite{foong2019between}. On the other hand, LL with large prior scale (>1e-2) suffers from under-fitting issue.}
    \label{fig:1d-tanh_hparams}
\end{figure*}

==> fig/1d_tanh_priors_cl.tex <==
\begin{figure*}[!h]
    \centering
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_tanh_priors_cl/0.1.pdf}
        \captionsetup{justification=centering}
        \caption{CL / TanH (1e-1)}
        \label{fig:cl_tanh_1e-1}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_tanh_priors_cl/1.0.pdf}
        \captionsetup{justification=centering}
        \caption{CL / TanH (1e-0)}
        \label{fig:cl_tanh_1e-0}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_tanh_priors_cl/10.0.pdf}
        \captionsetup{justification=centering}
        \caption{CL / TanH (1e+1)}
        \label{fig:cl_tanh_1e+1}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_tanh_priors_cl/100.0.pdf}
        \captionsetup{justification=centering}
        \caption{CL / TanH (1e+2)}
        \label{fig:cl_tanh_1e+2}
    \end{subfigure}
    \caption{Toy 1D regression task for Connectivity Laplace (CL) for various prior scales. While CL with small prior scale (<=1e-1) fail to capture 'in-between' uncertainty\cite{foong2019between}, CL with large prior scale (>1e-1) does not suffer from under-fitting issue.}
    \label{fig:1d-tanh_hparams_cl}
\end{figure*}

==> fig/1d_tanh_sigma.tex <==
\begin{figure*}[!h]
    \centering
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_tanh_sigma/0.001.pdf}
        \captionsetup{justification=centering}
        \caption{LL / TanH (1e-3)}
        \label{fig:ll_tanh_1e-3_sigma}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_tanh_sigma/0.01.pdf}
        \captionsetup{justification=centering}
        \caption{LL / TanH (1e-2)}
        \label{fig:ll_tanh_1e-2_sigma}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_tanh_sigma/0.1.pdf}
        \captionsetup{justification=centering}
        \caption{LL / TanH (1e-1)}
        \label{fig:ll_tanh_1e-1_sigma}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_tanh_sigma/1.0.pdf}
        \captionsetup{justification=centering}
        \caption{LL / TanH (1e-0)}
        \label{fig:ll_tanh_1e-0_sigma}
    \end{subfigure}
    \caption{Toy 1D regression task for Linearized Laplace (LL) for various prior scales. Results show that LL with small prior scale (1e-3) fails to capture 'in-between' uncertainty \cite{foong2019between}. On the other hand, LL with large prior scale (>=1e-2) suffers from under-fitting issue.}
    \label{fig:1d-tanh_sigma}
\end{figure*}

==> fig/1d_tanh_sigma_cl.tex <==
\begin{figure*}[!h]
    \centering
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_tanh_sigma_cl/0.1.pdf}
        \captionsetup{justification=centering}
        \caption{CL / TanH (1e-1)}
        \label{fig:cl_tanh_1e-1_sigma}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_tanh_sigma_cl/1.0.pdf}
        \captionsetup{justification=centering}
        \caption{CL / TanH (1e-0)}
        \label{fig:cl_tanh_1e-0_sigma}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_tanh_sigma_cl/10.0.pdf}
        \captionsetup{justification=centering}
        \caption{CL / TanH (1e+1)}
        \label{fig:cl_tanh_1e+1_sigma}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/1d_tanh_sigma_cl/100.0.pdf}
        \captionsetup{justification=centering}
        \caption{CL / TanH (1e+2)}
        \label{fig:cl_tanh_1e+2_sigma}
    \end{subfigure}
    \caption{Toy 1D regression task for Connectivity Laplace (CL) for various prior scales. While CL with small prior scale (<=1e-1) fail to capture 'in-between' uncertainty\cite{foong2019between}, CL with large prior scale (>1e-1) does not suffer from under-fitting issue.}
    \label{fig:1d-tanh_hparams_cl}
\end{figure*}

==> fig/2d_cls.tex <==
\begin{figure*}[!t]
    \centering
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/2d_cls/ntkgp_wo.pdf}
        \captionsetup{justification=centering}
        \caption{LL w.o. weight decay}
        \label{fig:local-ntkgp-wo-wd}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/2d_cls/ntkgp_w.pdf}
        \captionsetup{justification=centering}
        \caption{LL w. weight decay}
        \label{fig:local-ntkgp-w-wd}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/2d_cls/ctkgp_wo.pdf}
        \captionsetup{justification=centering}
        \caption{CL w.o. weight decay}
        \label{fig:local-ctkgp-wo-wd}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/2d_cls/ctkgp_w.pdf}
        \captionsetup{justification=centering}
    \caption{CL w. weight decay}
        \label{fig:local-ctkgp-w-wd}
    \end{subfigure}
    \caption{\footnotesize Uncertainty results of networks trained on 2D circle dataset with/without weight decay. We plot two classes of training data as green/blue circles. Bright color indicates high certainty, while dark color indicates high uncertainty.}
    \label{fig:2d-cls}
    \vspace{-0.5cm}
\end{figure*}

==> fig/2d_cls_tanh.tex <==
\begin{figure*}[!h]
    \centering
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/2d_cls_tanh/ntkgp_wo.pdf}
        \captionsetup{justification=centering}
        \caption{LL w.o. weight decay}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/2d_cls_tanh/ntkgp_w.pdf}
        \captionsetup{justification=centering}
        \caption{LL w. weight decay}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/2d_cls_tanh/ctkgp_wo.pdf}
        \captionsetup{justification=centering}
        \caption{CL w.o. weight decay}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/2d_cls_tanh/ctkgp_w.pdf}
        \captionsetup{justification=centering}
    \caption{CL w. weight decay}
    \end{subfigure}
    \caption{Uncertainty results of networks trained on 2D circle dataset with/without weight decay for TanH activation function. We plot two classes of training data as green/blue circles. Bright color indicates high certainty, while dark color indicates high uncertainty.}
    \vspace{-0.5cm}
\end{figure*}

==> fig/2d_cls_wo_bn.tex <==
\begin{figure*}[!h]
    \centering
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/2d_cls_wo_bn/ntkgp_wo.pdf}
        \captionsetup{justification=centering}
        \caption{LL w.o. weight decay}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/2d_cls_wo_bn/ntkgp_w.pdf}
        \captionsetup{justification=centering}
        \caption{LL w. weight decay}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/2d_cls_wo_bn/ctkgp_wo.pdf}
        \captionsetup{justification=centering}
        \caption{CL w.o. weight decay}
    \end{subfigure}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{fig/2d_cls_wo_bn/ctkgp_w.pdf}
        \captionsetup{justification=centering}
    \caption{CL w. weight decay}
    \end{subfigure}
    \caption{Uncertainty results of networks trained on 2D circle dataset with/without weight decay without BN. We plot two classes of training data as green/blue circles. Bright color indicates high certainty, while dark color indicates high uncertainty.}
\end{figure*}

==> fig/alpha.tex <==
\begin{figure*}[!t]
    \begin{subfigure}[t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{fig/alpha/alpha_NLL.pdf}
        \captionsetup{justification=centering}
        \caption{NLL}
        \label{fig:step_10}
    \end{subfigure}
    \begin{subfigure}[t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{fig/alpha/alpha_ECE.pdf}
        \captionsetup{justification=centering}
        \caption{ECE}
        \label{fig:step_0}
    \end{subfigure}
    \begin{subfigure}[t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{fig/alpha/alpha_Brier.pdf}
        \captionsetup{justification=centering}
        \caption{Brier Score}
        \label{fig:step_100}
    \end{subfigure}
    \caption{\footnotesize Sensitivity to $\alpha$. Expected calibration error (ECE), Negative Log-likelihood (NLL), and Brier score results on corrupted CIFAR-100 for ResNet-18. Showing the mean (line) and standard deviation (shaded area) across four different seeds.}
    \label{fig:alpha}
    \vspace{-0.5cm}
\end{figure*}

==> fig/corruption.tex <==
\begin{figure*}[!ht]
    \begin{subfigure}[t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{fig/corruption/Corruption_ECE.pdf}
        \captionsetup{justification=centering}
        \caption{ECE}
    \end{subfigure}
    \begin{subfigure}[t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{fig/corruption/Corruption_LL.pdf}
        \captionsetup{justification=centering}
        \caption{Log-Likelihood}
    \end{subfigure}
    \begin{subfigure}[t]{0.33\linewidth}
        \includegraphics[width=\linewidth]{fig/corruption/Corruption_Brier.pdf}
        \captionsetup{justification=centering}
        \caption{Brier Score}
    \end{subfigure}
    \caption{Expected calibration error (ECE), log-likelihood, and Brier score results on corrupted CIFAR-10 for ResNet-18 with MixUp. Showing the mean (line) and standard deviation (shaded area) across four different seeds.}
    \label{fig:corruption}
    \vspace{-0.5cm}
\end{figure*}

==> table/bound_ctk.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{\footnotesize Results for experiments on PAC-Bayes-CTK estimation.}
\label{tab:bound_ctk}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}c|cccc|cccc@{}}
\toprule
                & \multicolumn{4}{c|}{CIFAR-10}         & \multicolumn{4}{c}{CIFAR-100}         \\ \midrule
Parameter scale & 0.5     & 1.0     & 2.0     & 4.0     & 0.5     & 1.0     & 2.0     & 4.0     \\ \toprule
$\mathrm{tr}(\mathbf{C}^{\theta^*}_{\mathcal{X}})$ & 14515.0039      & 14517.7793      & 14517.3506      & 14518.4746      & 12872.6895      & 12874.4395      & 12873.9512      & 12875.541       \\
Bias            & 13.9791 & 13.4685 & 13.3559 & 13.3122 & 25.3686 & 24.8064 & 24.9102 & 24.7557 \\
Sharpness       & 24.6874 & 24.6938 & 24.6926 & 24.6941 & 26.0857 & 26.0894 & 26.0874 & 26.0916 \\
KL         & 19.3332 & 19.0812 & 19.0243 & 19.0032 & 25.7271 & 25.4479 & 25.4988 & 25.4236 \\ 
Test err.    & 0.0468 ± 0.0014 & 0.0463 ± 0.0013 & 0.0462 ± 0.0012 & 0.0460 ± 0.0013 & 0.2257 ± 0.0020 & 0.2252 ± 0.0017 & 0.2256 ± 0.0015 & 0.2253 ± 0.0017 \\ \midrule
PAC-Bayes-CTK       & 0.0918 ± 0.0013 & 0.0911 ± 0.0011 & 0.0909 ± 0.0011 & 0.0907 ± 0.0009 & 0.2874 ± 0.0034 & 0.2862 ± 0.0031 & 0.2860 ± 0.0032 & 0.2862 ± 0.0032 \\ \bottomrule
\end{tabular}
}
\vspace{-0.5cm}
\end{table}

==> table/bound_ntk.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[!h]
\centering
\caption{Results for experiments on PAC-Bayes-NTK estimation.}
\label{tab:bound_ntk}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}c|cccc|cccc@{}}
\toprule
                & \multicolumn{4}{c|}{CIFAR-10}             & \multicolumn{4}{c}{CIFAR-100}             \\ \midrule
Parameter scale & 0.5      & 1.0      & 2.0      & 4.0      & 0.5      & 1.0      & 2.0      & 4.0      \\ \toprule
$\mathrm{tr}(\Theta^{\theta^*}_{\mathcal{X}})$ & 18746194.0      & 6206303.5       & 3335419.75      & 2623873.25      & 12688970.0      & 3916139.25      & 2819272.5       & 2662497.0       \\
Bias            & 483.86   & 427.0042 & 299.0085 & 197.3149 & 476.9061 & 478.1776 & 440.284  & 329.8767 \\
Sharpness       & 579.6815 & 472.0    & 402.8186 & 369.3761 & 547.2874 & 434.7583 & 398.5075 & 387.3265 \\
KL divergence        & 531.7708 & 449.5021 & 350.9135 & 283.3455 & 512.0967 & 456.4679 & 419.3957 & 358.6016 \\
Test err.    & 0.5617 ± 0.0670 & 0.4566 ± 0.0604 & 0.2824 ± 0.0447 & 0.1530 ± 0.0199 & 0.6210 ± 0.0096 & 0.6003 ± 0.0094 & 0.5499 ± 0.0100 & 0.4666 ± 0.0093 \\ \midrule
PAC-Bayes-NTK       & 0.7985 ± 0.0694 & 0.6730 ± 0.0626 & 0.4718 ± 0.0465 & 0.3186 ± 0.0202 & 0.8530 ± 0.0140 & 0.8162 ± 0.0136 & 0.7602 ± 0.0112 & 0.6617 ± 0.0114 \\ \bottomrule
\end{tabular}
}
\end{table}

==> table/bounds.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Comparison of PAC-Bayes bound changes on function preserving scale transformation with VGG-13~\cite{Simonyan15} on CIFAR-100~\cite{krizhevsky2009learning} with MixUp.}
\label{tab:bounds}
{%
\begin{tabular}{@{}ccccc@{}}
\toprule
$k$ & PO~\cite{neyshabur2017exploring} & SAM~\cite{foret2020sharpness} & ASAM~\cite{kwon2021asam} & Ours \\ \midrule
1.0 & 1.000 & 1.000 & 1.000 & 1.000 \\
2.0 & 0.521 & 1.662 & 1.661 & 1.073 \\
4.0 & 0.601 & 3.127 & 3.111 & 1.087 \\
8.0 & 0.847 & 6.107 & 5.981 & 1.084 \\ \bottomrule
\end{tabular}%
}
\end{table}

==> table/cifar10-0.0-vgg.tex <==
\begin{table*}[!ht]
\caption{\footnotesize Uncertainty calibration results on CIFAR-10~\citep{krizhevsky2009learning} for VGG-13~\citep{Simonyan15}.}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccc}
\toprule
& \multicolumn{4}{c}{CIFAR-10}           \\ 
\midrule
&NLL~($\downarrow$)&ECE~($\downarrow$)&Brier.~($\downarrow$)&AUC~($\uparrow$) \\
\midrule

Deterministic & 0.4086 ± 0.0018	 & 0.0490 ± 0.0003 & 0.1147 ± 0.0005 & -\\
MCDO & 0.3889 ± 0.0049 & 0.0465 ± 0.0009 & 0.1106 ± 0.0015 & 0.7765 ± 0.0221 \\
MCBN & 0.3852 ± 0.0012 & 0.0462 ± 0.0002 & 0.1108 ± 0.0003 & 0.9051 ± 0.0065 \\
Batch Ensemble & 0.3544 ± 0.0036 & 0.0399 ± 0.0009 & 0.1064 ± 0.0012 & 0.9067 ± 0.0030 \\
Deep Ensemble & 0.2243 & 0.0121 & 0.0776 & 0.7706 \\\midrule
Linearized Laplace & 0.3366 ± 0.0013 & 0.0398 ± 0.0004 & 0.1035 ± 0.0003 & 0.8883 ± 0.0017 \\
Connectivity Laplace (Ours) & 0.2674 ± 0.0028 & 0.0234 ± 0.0011 & 0.0946 ± 0.0010 & 0.9002 ± 0.0033\\
\bottomrule 
\end{tabular}
}
\end{table*}

==> table/cifar10-0.0.tex <==
\begin{table*}[!ht]
\caption{\footnotesize Uncertainty calibration results on CIFAR-10~\citep{krizhevsky2009learning} for ResNet-18~\citep{he2016deep}.}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccc}
\toprule
& \multicolumn{4}{c}{CIFAR-10}           \\ 
\midrule
&NLL~($\downarrow$)&ECE~($\downarrow$)&Brier.~($\downarrow$)&AUC~($\uparrow$) \\
\midrule

Deterministic & 0.3135 ± 0.0088 & 0.0350 ± 0.0014 & 0.0875 ± 0.0026 & -\\
MCDO & 0.2845 ± 0.0148 & 0.0157 ± 0.0012 & 0.1056 ± 0.0062 & 0.9172 ± 0.0074 \\
MCBN & 0.2922 ± 0.0074 & 0.0325 ± 0.0010 & 0.0838 ± 0.0022 & 0.9431 ± 0.0033 \\
Batch Ensemble & 0.2740 ± 0.0030 & 0.0286 ± 0.0005 & 0.0814 ± 0.0009 & 0.9376 ± 0.0036 \\
Deep Ensemble & 0.1753 & 0.0067 & 0.0594 & 0.8527 \\\midrule
Linearized Laplace & 0.2077 ± 0.0032 & 0.0180 ± 0.0009 & 0.0816 ± 0.0010 & 0.8991 ± 0.0198 \\
Connectivity Laplace (Ours) & 0.2089 ± 0.0023 & 0.0120 ± 0.0019 & 0.0720 ± 0.0011 & 0.9705 ± 0.0098\\
\bottomrule 
\end{tabular}
}
\end{table*}

==> table/cifar10-0.4-vgg.tex <==
\begin{table*}[!ht]
\caption{Uncertainty calibration results on CIFAR-10~\cite{krizhevsky2009learning} for VGG-13~\cite{Simonyan15} with MixUp~\cite{zhang2018mixup}.}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccc}
\toprule
& \multicolumn{4}{c}{CIFAR-10}           \\ 
\midrule
&NLL~($\downarrow$)&ECE~($\downarrow$)&Brier.~($\downarrow$)&AUC~($\uparrow$) \\
\midrule

Deterministic & 0.3588 ± 0.0017 & 0.0418 ± 0.0002 & 0.1005 ± 0.0005 & -\\
MCDO \cite{gal2016dropout} & 0.3449 ± 0.0039 & 0.0404 ± 0.0006 & 0.0985 ± 0.0013 & 0.7728 ± 0.0171 \\
MCBN \cite{teye2018bayesian} & 0.3363 ± 0.0041&	0.0388 ± 0.0007&	0.0963 ± 0.0011&	0.9053 ± 0.0067 \\
Batch Ensemble \cite{wen2020batchensemble} & 0.3304 ± 0.0029&	0.0362 ± 0.0009&	0.0990 ± 0.0009&	0.9108 ± 0.0036 \\
Deep Ensemble \cite{lakshminarayanan2017deep} & 0.1867&	0.0078&	0.0660&	0.7902 \\\midrule
Linearized Laplace \cite{foong2019between} & 0.2849 ± 0.0028&	0.0316 ± 0.0006&	0.0888 ± 0.0007&	0.9032 ± 0.0037 \\
Connectivity Laplace (Ours) & 0.2315 ± 0.0021&	0.0169 ± 0.0005&	0.0824 ± 0.0002&	0.9092 ± 0.0045\\
\bottomrule 
\end{tabular}
}
\end{table*}

==> table/cifar10-0.4.tex <==
\begin{table*}[!ht]
\caption{Uncertainty calibration results on CIFAR-10~\cite{krizhevsky2009learning} for ResNet-18~\cite{he2016deep} with MixUp~\cite{zhang2018mixup}.}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccc}
\toprule
& \multicolumn{4}{c}{CIFAR-10}           \\ 
\midrule
& NLL~($\downarrow$)    & ECE~($\downarrow$) & Brier.~($\downarrow$) & AUC~($\uparrow$) \\
\midrule
Deterministic& 0.2750 ± 0.0009 & 0.0297 ± 0.0002 & 0.0765 ± 0.0003 & -\\
MCDO \cite{gal2016dropout} & 0.2060 ± 0.0032 & 0.0118 ± 0.0013 & 0.0737 ± 0.0010 & 0.9263 ± 0.0033 \\
MCBN \cite{teye2018bayesian} & 0.2560 ± 0.0021 & 0.0270 ± 0.0003 & 0.0725 ± 0.0007 & 0.9586 ± 0.0077\\
Batch Ensemble \cite{wen2020batchensemble} & 0.2512 ± 0.0044 & 0.0253 ± 0.0007 & 0.0741 ± 0.0011 & 0.9612 ± 0.0063\\
Deep Ensemble \cite{lakshminarayanan2017deep} & 0.1596 & 0.0070 & 0.0538 & 0.8956 \\\midrule
Linearized Laplace \cite{foong2019between} & 0.1647 ± 0.0021 & 0.0099 ± 0.0011 & 0.0689 ± 0.0015 & 0.9412 ± 0.0256 \\
Connectivity Laplace (Ours) & 0.1643 ± 0.0022 & 0.0046 ± 0.0007 & 0.0634 ± 0.0008 & 0.9712 ± 0.0086 \\
\bottomrule 
\end{tabular}}
\end{table*}

==> table/cifar100-0.0-vgg.tex <==
\begin{table*}[!ht]
\caption{\footnotesize Uncertainty calibration results on CIFAR-100 \citep{krizhevsky2009learning} for VGG-13 \citep{Simonyan15}.}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccc}
\toprule
& \multicolumn{4}{c}{CIFAR-100}           \\ 
\midrule
&NLL~($\downarrow$)&ECE~($\downarrow$)&Brier.~($\downarrow$)&AUC~($\uparrow$) \\
\midrule

Deterministic & 1.8286 ± 0.0066&	0.1544 ± 0.0010&	0.4661 ± 0.0018	 & -\\
MCDO & 1.7439 ± 0.0089&	0.1363 ± 0.0008&	0.4456 ± 0.0017&	0.6424 ± 0.0099 \\
MCBN & 1.7491 ± 0.0075	&0.1399 ± 0.0010	&0.4488 ± 0.0015	&0.7039 ± 0.0197 \\
Batch Ensemble & 1.6142 ± 0.0101	&0.1077 ± 0.0020	&0.4143 ± 0.0027	&0.7232 ± 0.0021 \\
Deep Ensemble & 1.2006	&0.0456	&0.3228	&0.6929 \\\midrule
Linearized Laplace & 1.5806 ± 0.0054	&0.1036 ± 0.0004	&0.4127 ± 0.0010	&0.6893 ± 0.0221 \\
Connectivity Laplace (Ours) & 1.4073 ± 0.0039	&0.0703 ± 0.0028	&0.3827 ± 0.0012	&0.7254 ± 0.0136\\
\bottomrule 
\end{tabular}
}
\end{table*}

==> table/cifar100-0.0.tex <==
\begin{table*}[t]
\caption{\footnotesize Uncertainty calibration results on CIFAR-100~\citep{krizhevsky2009learning} for ResNet-18~\citep{he2016deep}}\label{table:resnet-18-cifar-100}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccc}
\toprule
& \multicolumn{4}{c}{CIFAR-100}           \\ 
\midrule
&NLL~($\downarrow$)&ECE~($\downarrow$)&Brier.~($\downarrow$)&AUC~($\uparrow$) \\
\midrule
Deterministic& 1.5370 ± 0.0117 & 0.1115 ± 0.0017 & 0.3889 ± 0.0031 & -\\
MCDO & 1.4264 ± 0.0110 & 0.0651 ± 0.0008 & 0.3925 ± 0.0020 & 0.6907 ± 0.0121 \\
MCBN & 1.4689 ± 0.0106 & 0.0998 ± 0.0016 & 0.3750 ± 0.0028 & 0.7982 ± 0.0210 \\
Batch Ensemble & 1.4029 ± 0.0031 & 0.0842 ± 0.0005 & 0.3582 ± 0.0010 & 0.7887 ± 0.0115 \\
Deep Ensemble & 1.0110 & 0.0507 & 0.2740 & 0.7802 \\\midrule
Linearized Laplace & 1.1673 ± 0.0093 & 0.0632 ± 0.0010 & 0.3597 ± 0.0020 &  0.8066 ± 0.0120 \\
Connectivity Laplace (Ours) & 1.1307 ± 0.0042 & 0.0524 ± 0.0009 & 0.3319 ± 0.0005 & 0.8423 ± 0.0204 \\
\bottomrule 
\end{tabular}
}
\end{table*}

==> table/cifar100-0.4-vgg.tex <==
\begin{table*}[!ht]
\caption{Uncertainty calibration results on CIFAR-100~\cite{krizhevsky2009learning} for VGG-13~\cite{Simonyan15} with MixUp~\cite{zhang2018mixup}.}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccc}
\toprule
& \multicolumn{4}{c}{CIFAR-100}           \\ 
\midrule
&NLL~($\downarrow$)&ECE~($\downarrow$)&Brier.~($\downarrow$)&AUC~($\uparrow$) \\
\midrule

Deterministic & 1.8043 ± 0.0052	&0.1509 ± 0.0008	&0.4597 ± 0.0014 & -\\
MCDO \cite{gal2016dropout} & 1.7016 ± 0.0061	&0.1291 ± 0.0011	&0.4344 ± 0.0014	&0.6612 ± 0.0254 \\
MCBN \cite{teye2018bayesian} & 1.7181 ± 0.0055	&0.1356 ± 0.0011	&0.4400 ± 0.0014	&0.7792 ± 0.0272 \\
Batch Ensemble \cite{wen2020batchensemble} & 1.6364 ± 0.0112	&0.1100 ± 0.0017	&0.4204 ± 0.0023	&0.6945 ± 0.0287 \\
Deep Ensemble \cite{lakshminarayanan2017deep} & 1.1989	&0.0490	&0.3227	&0.6984 \\\midrule
Linearized Laplace \cite{foong2019between} &1.5616 ± 0.0039	&0.1009 ± 0.0010	&0.4084 ± 0.0012	&0.7186 ± 0.0064 \\
Connectivity Laplace (Ours) & 1.3836 ± 0.0039	&0.0718 ± 0.0007	&0.3777 ± 0.0012&	0.7368 ± 0.0032\\
\bottomrule 
\end{tabular}
}
\end{table*}

==> table/cifar100-0.4.tex <==
\begin{table*}[!t]
\caption{\footnotesize Uncertainty calibration results on CIFAR-100~\citep{krizhevsky2009learning} for ResNet-18~\citep{he2016deep}}\label{table:resnet-18-cifar-100-mixup}
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{c|cccc}
\toprule
& \multicolumn{4}{c}{CIFAR-100}           \\ 
\midrule
&NLL~($\downarrow$)&ECE~($\downarrow$)&Brier.~($\downarrow$)&AUC~($\uparrow$) \\
\midrule

Deterministic&1.4699 ± 0.0077 & 0.1018 ± 0.0011 & 0.3713 ± 0.0020 & -\\
MCDO & 1.2568 ± 0.0085 & 0.0592 ± 0.0007 & 0.3445 ± 0.0037 & 0.6907 ± 0.0121 \\
MCBN & 1.3855 ± 0.0073 & 0.0882 ± 0.0010 & 0.3537 ± 0.0016 & 0.8185 ± 0.0363 \\
Batch Ensemble & 1.3431 ± 0.0128 & 0.0739 ± 0.0016 & 0.3437 ± 0.0035 & 0.8258 ± 0.0258 \\
Deep Ensemble & 0.9735 & 0.0475 & 0.2659 & 0.7305 \\\midrule
Linearized Laplace & 1.0912 ± 0.0059 & 0.0713 ± 0.0012 & 0.3354 ± 0.0012 & 0.8781 ± 0.0216 \\
Connectivity Laplace (Ours) & 1.0693 ± 0.0111 & 0.0513 ± 0.0021 & 0.3126 ± 0.0028 & 0.8935 ± 0.0186 \\
\bottomrule 
\end{tabular}
}
\vspace{-0.3cm}
\end{table*}

==> table/sharpnes-generalization.tex <==
\begin{table}[t]
\centering
% \caption{Correlation analysis of sharpness measures with generalization gap. tr($\mathbf{H}$), tr($\mathbf{F}$), tr($\mathbf{\Theta}$) are the trace of Hessian, trace of Fisher information matrix and trace of empirical NTK at local optima (=tr($\hat{\Theta}_{\mathcal{XX}}^{\theta^*}$)), respectively. SO, PO, SM, PM are the abbreviation of sharpness-orig, pacbayes-orig, $1/\alpha'$ sharpness mag, and $1/\sigma'$ pacbayes mag, respectively. These measures are detailed in eq. 52, 49, 62, 61 in \citet{jiang2020fantastic}. AS and FR are the abbreviation of adaptive sharpness \cite{kwon2021asam} and Fisher-Rao metric \cite{liang2019fisher}, respectively. $\tau$ is the Kendall rank-correlation coefficient and each row with hyper-parameter name presents the granulated correlation coefficients of corresponding hyper-parameter. $\mathcal{K}$ represents the conditional mutual information between sharpness measure and generalization gap.}
\caption{\footnotesize Correlation analysis of sharpness measures with generalization gap. We refer Sec. \ref{subsec:gen-metric} for the details of sharpness measures (row) and correlation metrics for sharpness-generalization relationship (column).}
\label{table:sharpness}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{@{}cccccccccc|c@{}}
\toprule
 & tr($\mathbf{H}$) & tr($\mathbf{F}$) & tr($\mathbf{\Theta}^{\theta^*}$) & SO & PO & SM & PM & AS & FR & CS \\ \midrule
$\tau$ (rank corr.) & 0.706 & 0.679 & 0.703 & 0.490 & 0.436 & 0.473 & 0.636 & 0.755 & 0.649 & \textbf{0.837} \\\midrule
network depth & 0.764 & 0.652 & \textbf{0.978} & -0.358 & -0.719 & 0.774 & 0.545 & 0.756 & 0.771 & \textbf{0.978} \\
network width & 0.687 & 0.922 & 0.330 & -0.533 & -0.575 & 0.495 & 0.564 & 0.827 & 0.921 & \textbf{0.978} \\
mini-batch size & 0.976 & 0.810 & \textbf{0.988} & 0.859 & 0.893 & 0.909 & 0.750 & 0.829 & 0.685 & 0.905 \\
learning rate & 0.966 & 0.713 & \textbf{1.000} & 0.829 & 0.874 & 0.057 & 0.621 & 0.794 & 0.565 & 0.897 \\
weight decay & -0.031 & -0.103 & 0.402 & 0.647 & 0.711 & 0.168 & 0.211 & 0.710 & 0.373 & \textbf{0.742} \\\midrule
$\Psi$ (avg.) & 0.672 & 0.599 & 0.739 & 0.289 & 0.237 & 0.481 & 0.538 & 0.783 & 0.663 & \textbf{0.900} \\\midrule
$\mathcal{K}$ (cond. MI) & 0.320 & 0.243 & 0.352 & 0.039 & 0.041 & 0.049 & 0.376 & 0.483 & 0.288 & \textbf{0.539} \\ \bottomrule
\end{tabular}%
}
\vspace{-0.5cm}
\end{table}

% \begin{table*}[!t]
% \centering
% \caption{Correlation analysis of sharpness measures with generalization gap. tr($\mathbf{H}$), tr($\mathbf{F}$), tr($\mathbf{\Theta}$) are the trace of Hessian, trace of Fisher information matrix and trace of empirical NTK at local optima (=tr($\hat{\Theta}_{\mathcal{XX}}^{\theta^*}$)), respectively. SO, PO, SM, PM, AS are the abbreviation of sharpness-orig, pacbayes-orig, $1/\alpha'$ sharpness mag, $1/\sigma'$ pacbayes mag, and adaptive sharpness \cite{kwon2021asam}, respectively, and these measures are detailed in eq. 52, 49, 62, 61 in \citet{jiang2020fantastic}. $\tau$ is the Kendall rank-correlation coefficient and each row with hyper-parameter name presents the granulated correlation coefficients of corresponding hyper-parameter. $\mathcal{K}$ represents the conditional mutual information between sharpness measure and generalization gap.}
% \begin{tabular}{c|ccccccccc}
% \hline
% & tr($\mathbf{H}$)  & tr($\mathbf{F}$)  & tr($\mathbf{\Theta}$) & CS & SO & PO & SM & PM & AS\\
% \hline
% $\tau$ (rank corr.) & 0.706 & 0.679 & 0.703 & \textbf{0.837} & 0.490 & 0.436 & 0.473 & 0.636 & 0.755\\
% \hline
% network depth       & 0.764 & 0.652 & \textbf{0.978} & \textbf{0.978} & -0.358 & -0.719 & 0.774 & 0.545 & 0.756 \\
% network width       & 0.687 & 0.922 & 0.330 & \textbf{0.978} & -0.533 & -0.575 & 0.495 & 0.564 & 0.827\\
% mini-batch size     & 0.976 & 0.810 & \textbf{0.988} & 0.905 & 0.859 & 0.893 & 0.909 & 0.750 & 0.829 \\
% learning rate       & 0.966 & 0.713  & \textbf{1.000} & 0.897 & 0.829 & 0.874 & 0.057 & 0.621 & 0.794 \\
% weight decay        & -0.031 & -0.103 & 0.402 & \textbf{0.742} & 0.647 & 0.711 & 0.168 & 0.211 & 0.710 \\
% \hline
% $\Psi$ (avg.)       & 0.672  & 0.599  & 0.739 & \textbf{0.900} & 0.289 & 0.237 & 0.481 & 0.538 & 0.783 \\
% \hline
% $\mathcal{K}$ (cond. MI)  & 0.320  & 0.243  & 0.352 & \textbf{0.539} & 0.039 & 0.041 & 0.049 & 0.376 & 0.483                             
% \end{tabular}
% \label{table:sharpness}
% % \vspace{-0.5cm}
% \end{table*}

==> table/uci_orig.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{\footnotesize Test negative log-likelihood on two UCI variants~\citep{hernandez2015probabilistic, foong2019between}}
\label{tab:uci}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccccc|cccc@{}}
\toprule
 & \multicolumn{4}{c|}{Original \citep{hernandez2015probabilistic} } & \multicolumn{4}{c}{GAP variants \citep{foong2019between} } \\ \midrule
 & Deep Ensemble & MCDO & LL & CL & Deep Ensemble & MCDO & LL & CL \\ \midrule
boston\_housing & 2.90 ± 0.03 & 2.63 ± 0.01 & \textbf{2.85 ± 0.01} & 2.88 ± 0.02 & 2.71 ± 0.01 & 2.68 ± 0.01 & \textbf{2.74 ± 0.01} & 2.75 ± 0.01 \\
concrete\_strength & 3.06 ± 0.01 & 3.20 ± 0.00 & 3.22 ± 0.01 & \textbf{3.11 ± 0.02} & 4.03 ± 0.07 & 3.42 ± 0.00 & \textbf{3.47 ± 0.01} & 4.03 ± 0.02 \\
energy\_efficiency & 0.74 ± 0.01 & 1.92 ± 0.01 & 2.12 ± 0.01 & \textbf{0.83 ± 0.01} & 0.77 ± 0.01 & 1.78 ± 0.01 & 2.02 ± 0.01 & 0.90 ± 0.02 \\
kin8nm & -1.07 ± 0.00 & -0.80 ± 0.01 & -0.90 ± 0.00 & \textbf{-1.07 ± 0.00} & -0.94 ± 0.00 & -0.71 ± 0.00 & -0.87 ± 0.00 & \textbf{-0.93 ± 0.00} \\
naval\_propulsion & -4.83 ± 0.00 & -3.85 ± 0.00 & -4.57 ± 0.00 & \textbf{-4.76 ± 0.00} & -2.22 ± 0.33 & -3.36 ± 0.01 & -3.66 ± 0.11 & \textbf{-3.80 ± 0.07} \\
power\_plant & 2.81 ± 0.00 & 2.91 ± 0.00 & 2.91 ± 0.00 & \textbf{2.81 ± 0.00} & 2.91 ± 0.00 & 2.97 ± 0.00 & 2.98 ± 0.00 & \textbf{2.91 ± 0.00} \\
protein\_structure & 2.89 ± 0.00 & 2.96 ± 0.00 & 2.91 ± 0.00 & \textbf{2.89 ± 0.00} & 3.11 ± 0.00 & 3.07 ± 0.00 & \textbf{3.07 ± 0.00} & 3.13 ± 0.00 \\
wine & 1.21 ± 0.00 & 0.96 ± 0.01 & \textbf{1.24 ± 0.01} & 1.27 ± 0.01 & 1.48 ± 0.01 & 1.03 ± 0.00 & 1.45 ± 0.01 & \textbf{1.43 ± 0.00} \\
yacht\_hydrodynamics & 1.26 ± 0.04 & 2.17 ± 0.06 & \textbf{1.20 ± 0.04} & 1.25 ± 0.04 & 1.71 ± 0.03 & 3.06 ± 0.02 & 1.78 ± 0.02 & \textbf{1.74 ± 0.01} \\ \bottomrule
\end{tabular}%
}
\vspace{-0.5cm}
\end{table}
